X-ray spectral studies of TeV gamma-ray emitting blazars

This work is a summary of the X-ray spectral studies of 29 TeV $\gamma$-ray emitting blazars observed with Swift/XRT, especially focusing on sources for which X-ray regime allows to study the low and the high energy ends of the particle distributions function. Variability studies require simultaneous coverage, ideally sampling different flux states of each source. This is achieved using X-ray observations by disentangling the high-energy end of the synchrotron emission and the low-energy end of the Compton emission, which are produced by the same electron population. We focused on a sample of 29 TeV gamma-ray emitting blazars with the best signal-to-noise X-ray observations collected with Swift/XRT in the energy range of 0.3-10 keV during 10 years of Swift/XRT operations. We investigate the X-ray spectral shapes and the effects of different corrections for neutral hydrogen absorption and decompose the synchrotron and inverse Compton components. In the case of 5 sources (3C 66A, S5 0716+714, W Comae, 4C +21.35 and BL Lacertae) a superposition of both components is observed in the X-ray band, permitting simultaneous, time resolved studies of both ends of the electron distribution. The analysis of multi-epoch observations revealed that the break energy of X-ray spectrum varies only by a small factor with flux changes. Flux variability is more pronounced in the synchrotron domain (high-energy end of the electron distribution) than in the Compton domain (low energy end of the electron distribution). The spectral shape of the Compton domain is stable, while the flux of the synchrotron domain is variable. These changes cannot be described by simple variations of the cut-off energy, suggesting that the high-energy end of the electron distribution is not generally well-described by cooling only.

==> tables/bk_fits.tex <==
\begin{table*}

\caption{Fit parameters for the  \bk\ fits.  (1) The object
name, (2) source of \nh\ value, (3)-(6) the spectral indices, normalization and
break energy for the \bk\ fit defined in Sect.~3, (7) the reduced
$\chi^2$ value and the number of degrees of freedom.}

\label{table_fitpar_bk}

\begin{tabular}{rcccccc}
\hline
Object & N$_H$& $\Gamma_1$ & $\Gamma_2$ & $N_b$ & $E_{b}$ & $\chi_{red}^2$/n$_{d.o.f}$ \\
       &     &     &     &10$^{-2}$\,cm$^{-2}$\,s$^{-1}$\,keV$^{-1}$  & keV & \\
(1)    & (2) & (3) & (4) & (5) & (6) & (7)  \\

\hline
3C\,66A            & LAB  &2.462$\pm$0.017   &  1.746$\pm$0.170   &  0.139$\pm$0.001 &  3.383$\pm$0.328  & 0.949/260\\
                   & DL   &2.540$\pm$0.018   &  1.794$\pm$0.140   &  0.145$\pm$0.001 &  3.064$\pm$0.261  & 0.961/260\\
                   & Will &2.615$\pm$0.020   &  1.936$\pm$0.104   &  0.150$\pm$0.001 &  2.568$\pm$0.213  & 0.985/260\\
                   & free &2.470$\pm$0.040   &  1.739$\pm$0.168   &  0.140$\pm$0.001 &  3.372$\pm$0.340  & 0.952/259\\
\\
S5\,0716$+$714     & LAB  & 2.168$\pm$0.024  &  1.937$\pm$0.016   &  0.221$\pm$0.003 &  1.094$\pm$0.100 & 0.986/433\\
                   & DL   & 2.240$\pm$0.026  &  1.942$\pm$0.015   &  0.223$\pm$0.003 &  1.087$\pm$0.075 & 0.967/433\\
                   & Will & 2.213$\pm$0.025  &  1.940$\pm$0.015   &  0.223$\pm$0.003 &  1.092$\pm$0.082 & 0.973/433\\
                   & free & 2.511$\pm$0.085  &  1.965$\pm$0.017   &  0.231$\pm$0.002 &  1.046$\pm$0.042 & 0.942/432\\
\\
W\,Comae           & LAB  & 2.492$\pm$0.019  &  2.076$\pm$0.074   &  0.066$\pm$0.001 &  2.027$\pm$0.234 & 0.988/252\\
                   & DL   & 2.474$\pm$0.018  &  2.080$\pm$0.076   &  0.066$\pm$0.001 &  2.047$\pm$0.252 & 0.993/252\\
                   & Will & 2.504$\pm$0.019  &  2.070$\pm$0.071   &  0.669$\pm$0.001 &  2.028$\pm$0.218 & 0.986/252\\
                   & free & 2.538$\pm$0.050  &  2.071$\pm$0.069   &  0.677$\pm$0.001 &  1.976$\pm$0.212 & 0.987/251\\
\\
4C\,$+$21.35       & LAB  & 2.106$\pm$0.034  &  1.442$\pm$0.021   &  0.061$\pm$0.001 &  1.183$\pm$0.054 & 0.989/373\\
                   & DL   & 2.124$\pm$0.034  &  1.444$\pm$0.021   &  0.062$\pm$0.001 &  1.177$\pm$0.052 & 0.990/373\\
                   & Will & 2.128$\pm$0.034  &  1.444$\pm$0.021   &  0.616$\pm$0.001 &  1.176$\pm$0.052 & 0.991/373\\
                   & free & 1.978$\pm$0.093  &  1.432$\pm$0.022   &  0.604$\pm$0.001 &  1.222$\pm$0.071 & 0.987/372\\
\\
BL\,Lacertae       & LAB  & 1.155$\pm$0.023  &  1.705$\pm$0.014   &  0.260$\pm$0.002 &  1.611$\pm$0.048 & 1.173/614\\
                   & DL   & 1.374$\pm$0.021  &  1.728$\pm$0.016   &  0.286$\pm$0.002 &  1.766$\pm$0.081 & 1.122/614\\
                   & Will & 1.996$\pm$0.047  &  1.727$\pm$0.010   &  0.363$\pm$0.005 &  1.095$\pm$0.087 & 1.098/614\\
                   & free & 1.570$\pm$0.056  &  1.740$\pm$0.019   &  0.318$\pm$0.010 &  1.983$\pm$0.232 & 1.105/613\\
\hline

\end{tabular}
\end{table*}


==> tables/nh_compare.tex <==
\begin{table*}  

\caption[]{The comparison of Galactic column density values.  (1) The object
name, (2)-(5) the \nh\ values provided by \cite{Kalberla05},
\cite{Dickey90},\cite{Willingale13}, respectively,  (6)-(8) the free \nh\ value
obtained with the  \lp, the \po\ and the\bk\ model fitted.}
\label{table_nh}

\centering

\begin{tabular}{rccccccc}

\hline
 Object & N$_{H}^{LAB}$ & N$_{H}^{DL}$& N$_{H}^{H_2}$  &  N$_{H}^{Will}$ & N$_{H}^{LP,\mathit{free}}$ & N$_{H}^{PL,\mathit{free}}$ & N$_{H}^{BP ,\mathit{free}}$ \\
        &[10$^{20}$\,cm$^{-2}$]&[10$^{20}$\,cm$^{-2}$]&[10$^{20}$\,cm$^{-2}$]&[10$^{20}$\,cm$^{-2}$] &[10$^{20}$\,cm$^{-2}$]  & [10$^{20}$\,cm$^{-2}$] &  [10$^{20}$\,cm$^{-2}$]     \\
    (1)    & (2) & (3) & (4) & (5) & (6) & (7) & (8)\\
\hline
 
SHBL\,J001355.9$-$185406 & 2.13  & 2.09  & 0.17  & 2.30  && \\
KUV\,00311$-$1938        & 1.67  & 1.59  & 0.10  & 1.77  && \\
1ES\,0033$+$595          & 41.80 & 42.70 & 14.40 & 56.20 & 59.36$\pm$0.42 & 68.80$\pm$0.19 \\
RGB\,J0136$+$391         & 6.00  & 5.96  & 1.30  & 7.30  &12.0$\pm$1.5& 11.10$\pm$0.53 \\
RGB\,J0152$+$017         & 2.68  & 2.89  & 0.23  & 2.91  && \\
3C\,66A                  & 7.37  & 8.49  & 2.02  & 9.40  & 11.79$\pm$0.12 & 6.31$\pm$0.42  & 7.50$\pm$0.54 \\
1ES\,0229$+$200          & 8.06  & 9.20  & 3.69  & 11.80 & 7.86$\pm$1.98 & 13.19$\pm$0.81\\
PKS\,0301$-$243          & 1.70  & 1.82  & 0.10  & 1.79  && \\
IC\,310                  & 12.20 & 13.30 & 6.16  & 18.30 && \\
RBS\,0413                & 8.84  & 10.50 & 4.11  & 12.90 && \\
1ES\,0347$-$121          & 3.09  & 3.60  & 0.56  & 3.65  && \\
1ES\,0414$+$009          & 8.85  & 10.30 & 4.88  & 13.70 &&  \\
PKS\,0447$-$439          & 1.18  & 1.99  & 0.04  & 1.22  & 2.79$\pm$0.58 &  3.57$\pm$0.27 \\
1ES\,0502$+$675          & 9.37  & 9.56  & 5.16  & 14.50 & 15.61$\pm$1.35 & 16.37$\pm$0.46 \\
VER\,J0521$+$211         & 28.60 & 33.40 & 14.40 & 42.90 && \\
PKS\,0548$-$322          & 2.58  & 2.18  & 0.30  & 2.87  & 2.14$\pm$0.50 & 4.41$\pm$0.22  \\
RX\,J0648.7$+$1516       & 16.80 & 19.40 & 8.72  & 25.50 && \\
1ES\,0647$+$250          & 11.80 & 12.80 & 4.06  & 15.80 & 14.30$\pm$1.00 & 17.82$\pm$0.35 \\
RGB\,J0710$+$591         & 4.48  & 5.57  & 0.75  & 5.23  && \\
S5\,0716$+$714           & 3.22  & 3.82  & 0.39  & 3.60  & 3.96$\pm$0.54 & 1.92$\pm$0.22    & 6.04$\pm$0.66\\
1ES\,0806$+$524          & 4.16  & 4.45  & 0.73  & 4.89  & 5.45$\pm$0.78 & 7.11$\pm$0.34 \\
RBS\,0723                & 3.39  & 4.06  & 0.41  & 3.79  && \\
1RXS\,J101015.9$-$311909 & 7.90  & 7.36  & 2.33  & 10.20 && \\
S4\,0954+65              & 4.80  & 3.69  & 1.50  & 6.30 && \\
1ES\,1011$+$496          & 0.84  & 0.79  & 0.02  & 0.86  & 1.75$\pm$0.47 & 3.04$\pm$0.22  \\
1ES\,1101$-$232          & 5.51  & 5.63  & 1.39  & 6.90  & 3.67$\pm$1.12 & 6.36$\pm$0.49 \\
Markarian\,421           & 1.91  & 1.43  & 0.11  & 2.01  && \\
Markarian\,180           & 1.17  & 1.42  & 0.05  & 1.22  & 2.71$\pm$0.58 & 3.67$\pm$0.26\\
RX\,J1136.5$+$6737       & 1.03  & 1.33  & 0.03  & 1.06  &1.8$\pm$1.1&3.57$\pm$0.47 \\
1ES\,1215$+$303          & 1.70  & 1.68  & 0.09  & 1.80  && \\
1ES\,1218$+$304          & 1.99  & 1.75  & 0.13  & 2.12  & 1.00$\pm$0.80 & 3.05$\pm$0.37 \\
W\,Comae                 & 2.04  & 1.84  & 0.14  & 2.18  & 4.54$\pm$0.74 & 8.75$\pm$0.32   &  2.54$\pm$0.50\\ 
MS\,1221.8$+$2452        & 1.79  & 1.80  & 1.78  & 1.91  &4.55$\pm$0.98&5.73$\pm$0.43 \\
4C\,$+$21.35             & 2.12  & 2.26  & 0.17  & 2.29  & 0.48$\pm$0.64 &  0.00$\pm$0.00  & 1.07$\pm$0.73\\
S3\,1227+25              & 1.42  & 1.54  & 0.08  & 1.50 && \\
3C\,279                  & 2.01  & 2.21  & 0.21  & 2.22  & 1.58$\pm$0.44 &  3.74$\pm$0.20   \\
1ES\,1312$-$423          & 7.77  & 7.93  & 3.42  & 11.20 && \\
PKS\,1424$+$240          & 2.84  & 2.67  & 0.35  & 3.19  &6.63$\pm$0.74&6.25$\pm$0.32 \\
H\,1426$+$428            & 1.11  & 1.38  & 0.04  & 1.14  & 1.17$\pm$0.33 & 3.12$\pm$0.15 \\
1ES\,1440$+$122          & 1.58  & 1.61  & 0.14  & 1.72  && \\
PKS\,1441+25             & 3.12  & 2.68  & 0.37  & 3.49  && \\
PKS\,1510$-$089          & 6.99  & 7.80  & 2.46  & 9.45  & 5.09$\pm$0.60 & 5.28$\pm$0.25 \\
AP\,Librae               & 8.36  & 8.70  & 4.25  & 4.17  && \\
PG\,1553$+$113           & 3.67  & 3.69  & 0.68  & 4.35  & 4.71$\pm$0.46 & 5.03$\pm$0.20 \\
Markarian\,501           & 1.58  & 1.67  & 0.08  & 1.66  && \\
H\,1722$+$119            & 8.70  & 8.61  & 5.09  & 13.80 && \\
1ES\,1727$+$502          & 2.38  & 2.79  & 0.23  & 2.60  && \\
1ES\,1741$+$196          & 7.32  & 6.82  & 2.26  & 9.58  && \\
HESS\,J1943$+$213        & 82.40 & 88.10 & 14.40 & 96.80 && \\
1ES\,1959$+$650          & 9.83  & 10.30 & 6.06  & 15.90 & 11.17$\pm$0.80 & 15.11$\pm$0.31 \\
MAGIC\,J2001$+$435       & 37.00 & 43.10 & 14.40 & 51.40 && \\
PKS\,2005$-$489          & 3.94  & 5.04  & 0.72  & 4.66  & 3.91$\pm$0.57 & 3.54$\pm$0.25 \\
PKS\,2155$-$304          & 1.52  & 1.71  & 0.11  & 1.63  & 2.47$\pm$0.94 &  3.51$\pm$0.43 \\
BL\,Lacertae             & 18.30 & 21.60 & 12.00 & 30.30 & 24.77$\pm$1.16 & 27.59$\pm$0.46 & 25.09$\pm$1.02 \\
B3\,2247$+$381           & 10.20 & 12.20 & 5.16  & 15.40 &13.5$\pm$1.6&16.87$\pm$0.59 \\
RGB\,J2243+203           & 5.25  & 5.41  & 1.07  & 6.33  && \\
1ES\,2344$+$514          & 15.10 & 16.80 & 9.47  & 24.60 & 14.34$\pm$0.88 & 19.18$\pm$0.33  \\
H\,2356$-$309            & 1.42  & 1.32  & 0.06  & 1.48  && \\

\hline

\end{tabular}
\end{table*}


==> tables/po_fits.tex <==
%%%%%%%%%%%%%%%%%%
% PAGE 1
%%%%%%%%%%%%%%%%%%

\begin{table*}

\caption{Fit parameters for the power-law fits.  (1) The  object name, (2) source of \nh\ value, (3)-(4) the spectral index and the normalization for the \po\
fit defined in Sect.~3,   (5) the reduced $\chi^2$ value and the
number of degrees of freedom, (6) the test statistics value for F-test, (7)
probability, (8) preferred spectral model: PO - for the \po\ and LP - for the \lp\ model.}

\label{table_fitpar_po}

\centering

\begin{tabular}{rccccccc}

\hline
Object & N$_H$& $\Gamma$ & $N_p$ & $\chi_{red}^2$/n$_{d.o.f}$ &  F &  p-value & Model  \\
&  &    &10$^{-2}$\,cm$^{-2}$\,s$^{-1}$\,keV$^{-1}$ & &   & &\\
(1)    & (2) & (3) & (4) & (5) & (6)  & (7)  & (8) \\
\hline

1ES\,0033$+$595    & LAB  & 1.62$\pm$0.01 & 2.581$\pm$0.037 & 1.800/367& 264& 1$\cdot10^{-16}$ &  LP  \\
                   & DL   & 1.64$\pm$0.01 & 2.635$\pm$0.038 & 1.736/367& 244& 1$\cdot10^{-16}$ &  LP  \\
                   & Will & 1.84$\pm$0.02 & 3.476$\pm$0.052 & 1.143/367&  53& 1$\cdot10^{-12}$ &  LP  \\
                   & free & 1.99$\pm$0.03 & 4.322$\pm$0.151 & 1.013/366&   5& 0.02             &  PO  \\
\\
RGB\,J0136$+$391   & LAB  & 2.17$\pm$0.01 & 0.671$\pm$0.006 & 1.321/260& 114& 1$\cdot10^{-16}$ & LP  \\
                   & DL   & 2.17$\pm$0.01 & 0.670$\pm$0.006 & 1.329/260& 115& 1$\cdot10^{-16}$ & LP  \\
                   & Will & 2.23$\pm$0.01 & 0.711$\pm$0.007 & 1.094/260&  57& 1$\cdot10^{-13}$ & LP  \\
                   & free & 2.42$\pm$0.03 & 0.830$\pm$0.018 & 0.845/259& 0.7& 0.4              & PO  \\
\\
3C\,66A            & LAB  & 2.42$\pm$0.02 & 0.140$\pm$0.001 & 1.066/262&  21& 6$\cdot10^{-6}$  &  LP  \\
                   & DL   & 2.48$\pm$0.02 & 0.146$\pm$0.001 & 1.137/262&  49& 2$\cdot10^{-11}$ &  LP  \\
                   & Will & 2.53$\pm$0.02 & 0.151$\pm$0.001 & 1.223/262&  78& 1$\cdot10^{-16}$ &  LP  \\
                   & free & 2.36$\pm$0.03 & 0.134$\pm$0.003 & 1.047/261&  34& 1$\cdot10^{-8}$  &  LP  \\
\\
1ES\,0229$+$200    & LAB  & 1.59$\pm$0.02 & 0.370$\pm$0.005 & 1.381/266&  51 & 8$\cdot10^{-12}$ &  LP  \\
                   & DL   & 1.62$\pm$0.02 & 0.385$\pm$0.005 & 1.300/266&  32 & 4$\cdot10^{-8}$ &  LP  \\
                   & Will & 1.70$\pm$0.02 & 0.421$\pm$0.006 & 1.202/266&   6 & 0.01 &  PO  \\
                   & free & 1.74$\pm$0.03 & 0.441$\pm$0.013 & 1.194/265&   7 & 7$\cdot10^{-3}$ &  LP  \\
\\
PKS\,0447$-$439    & LAB  & 2.51$\pm$0.01 & 0.623$\pm$0.004 & 1.474/274&  70 & 3$\cdot10^{-15}$ &  LP  \\
                   & DL   & 2.57$\pm$0.01 & 0.647$\pm$0.004 & 1.285/274&  32& 4$\cdot10^{-8}$ &  LP  \\
                   & Will & 2.51$\pm$0.01 & 0.624$\pm$0.004 & 1.462/274&  67& 7$\cdot10^{-15}$ &  LP  \\
                   & free & 2.67$\pm$0.02 & 0.694$\pm$0.009 & 1.155/273&   2 & 0.2 &  PO  \\
\\
1ES\,0502$+$675    & LAB  & 2.05$\pm$0.01 & 1.227$\pm$0.009 & 1.885/349& 247 & 1$\cdot10^{-16}$ &  LP  \\
                   & DL   & 2.06$\pm$0.01 & 1.237$\pm$0.009 & 1.833/349& 228 & 1$\cdot10^{-16}$ &  LP  \\
                   & Will & 2.26$\pm$0.01 & 1.497$\pm$0.011 & 1.079/349&  17 & 5$\cdot10^{-5}$ &  LP  \\
                   & free & 2.33$\pm$0.02 & 1.597$\pm$0.028 & 1.031/348&   1 & 0.6 &  PO  \\
\\
PKS\,0548$-$322    & LAB  & 1.80$\pm$0.01 & 1.001$\pm$0.005 & 1.142/530& 104 & 1$\cdot10^{-16}$ &  LP  \\
                   & DL   & 1.78$\pm$0.01 & 0.984$\pm$0.005 & 1.216/530& 146 & 1.$\cdot10^{-16}$ &  LP  \\
                   & Will & 1.81$\pm$0.01 & 1.014$\pm$0.005 & 1.098/530&  78 & 1$\cdot10^{-16}$ &  LP  \\
                   & free & 1.87$\pm$0.01 & 1.080$\pm$0.011 & 1.000/529&  25 & 9$\cdot10^{-7}$ &  LP  \\
\\
1ES\,0647$+$250    & LAB  & 1.16$\pm$0.01 & 0.915$\pm$0.005 & 2.013/427& 328 & 1$\cdot10^{-16}$ &  LP  \\
                   & DL   & 2.20$\pm$0.01 & 0.952$\pm$0.005 & 1.729/427& 228 & 1$\cdot10^{-16}$ &  LP  \\
                   & Will & 2.32$\pm$0.01 & 1.062$\pm$0.006 & 1.236/427&  42 & 3$\cdot10^{-10}$ &  LP  \\
                   & free & 2.39$\pm$0.02 & 1.138$\pm$0.015 & 1.155/426&  12 & 5$\cdot10^{-4}$ &  LP  \\
\\
S5\,0716$+$714     & LAB  & 2.03$\pm$0.01 & 0.232$\pm$0.001 & 1.145/435&  50 & 6$\cdot10^{-12}$ &  LP  \\
                   & DL   & 2.06$\pm$0.01 & 0.237$\pm$0.001 & 1.228/435&  88 & 1$\cdot10^{-16}$ &  LP  \\
                   & Will & 2.05$\pm$0.01 & 0.235$\pm$0.001 & 1.195/435&  73 & 2$\cdot10^{-16}$ &  LP  \\
                   & free & 1.96$\pm$0.01 & 0.219$\pm$0.002 & 1.069/434&  19 & 1$\cdot10^{-5}$ &  LP  \\
\\
1ES\,0806$+$524    & LAB  & 2.42$\pm$0.01 & 0.393$\pm$0.003 & 1.316/285&  93 & 1$\cdot10^{-16}$ &  LP  \\
                   & DL   & 2.44$\pm$0.01 & 0.398$\pm$0.003 & 1.252/285&  76 & 2$\cdot10^{-16}$ &  LP  \\
                   & Will & 2.46$\pm$0.01 & 0.406$\pm$0.003 & 1.171/285&  55 & 2$\cdot10^{-12}$ &  LP  \\
                   & free & 2.59$\pm$0.02 & 0.446$\pm$0.007 & 1.003/284&   6 & 0.02 &  PO  \\
\\
1ES\,1011$+$496    & LAB  & 2.29$\pm$0.01 & 0.895$\pm$0.005 & 1.606/361&  97 & 1$\cdot10^{-16}$ &  LP  \\
                   & DL   & 2.29$\pm$0.01 & 0.892$\pm$0.005 & 1.622/361& 101 & 1$\cdot10^{-16}$ &  LP  \\
                   & Will & 2.29$\pm$0.01 & 0.895$\pm$0.005 & 1.600/361&  96 & 1$\cdot10^{-16}$ &  LP  \\
                   & free & 2.42$\pm$0.02 & 0.989$\pm$0.011 & 1.282/360&   7 & 7$\cdot10^{-3}$ &  LP  \\
\\
1ES\,1101$-$232    & LAB  & 2.06$\pm$0.01 & 1.880$\pm$0.019 & 1.057/270&   7 & 9$\cdot10^{-3}$ &  LP  \\
                   & DL   & 2.06$\pm$0.01 & 1.890$\pm$0.019 & 1.054/270&   6 & 0.01 &  PO  \\
                   & Will & 2.11$\pm$0.02 & 1.986$\pm$0.020 & 1.049/270&  -0.1 & 1 &  PO  \\
                   & free & 2.09$\pm$0.03 & 1.945$\pm$0.042 & 1.049/269&   6 & 0.01 &  PO  \\


\hline
\end{tabular}
\end{table*}

%%%%%%%%%%%%%%%%%%
% PAGE 2
%%%%%%%%%%%%%%%%%%

\clearpage
\newpage

\begin{table*}

\contcaption{}

%\label{table_fitpar_po}

\centering

\begin{tabular}{rccccccc}

\hline
(1)    & (2) & (3) & (4) & (5) & (6)  & (7)  & (8) \\
\hline

Mrk\,180           & LAB  & 2.15$\pm$0.01 & 0.808$\pm$0.005 & 1.326/240& -24 & 1 &  PO  \\
                   & DL   & 2.16$\pm$0.01 & 0.818$\pm$0.005 & 1.259/340&  87 & 1$\cdot10^{-16}$ &  LP  \\
                   & Will & 2.15$\pm$0.01 & 0.810$\pm$0.005 & 1.312/340& 102 & 1$\cdot10^{-16}$ &  LP  \\
                   & free & 2.28$\pm$0.02 & 0.905$\pm$0.011 & 0.999/339&   3 & 0.07 &  PO  \\
\\
RX\,J1136.5$+$6737 & LAB  & 1.73$\pm$0.01 & 0.401$\pm$0.004 & 1.171/272&  35 & 1$\cdot10^{-8}$ & LP  \\
                   & DL   & 1.75$\pm$0.01 & 0.407$\pm$0.004 & 1.141/272&  27 & 3$\cdot10^{-7}$ & LP  \\
                   & Will & 1.73$\pm$0.01 & 0.402$\pm$0.004 & 1.168/272&  34 & 1$\cdot10^{-8}$ & LP  \\
                   & free & 1.84$\pm$0.03 & 0.448$\pm$0.010 & 1.050/271&   3 & 0.1             & PO  \\
\\
1ES\,1218$+$304    & LAB  & 2.07$\pm$0.01 & 0.906$\pm$0.008 & 1.248/288&  13 & 4$\cdot10^{-4}$ &  LP  \\
                   & DL   & 2.06$\pm$0.01 & 0.896$\pm$0.008 & 1.264/288&  18 & 4$\cdot10^{-5}$ &  LP  \\
                   & Will & 2.08$\pm$0.01 & 0.911$\pm$0.008 & 1.240/288&  11 & 1$\cdot10^{-3}$ &  LP  \\
                   & free & 2.12$\pm$0.02 & 0.948$\pm$0.017 & 1.220/287&   7 & 0.01 &  LP  \\
\\
W\,Comae           & LAB  & 2.42$\pm$0.01 & 0.068$\pm$0.001 & 1.160/254&  37 & 4$\cdot10^{-9}$ &  LP  \\
                   & DL   & 2.41$\pm$0.01 & 0.067$\pm$0.001 & 1.144/254&  26 & 7$\cdot10^{-7}$ &  LP  \\
                   & Will & 2.43$\pm$0.01 & 0.068$\pm$0.001 & 1.172/254&  42& 5$\cdot10^{-10}$ &  LP  \\
                   & free & 2.34$\pm$0.03 & 0.065$\pm$0.001 & 1.113/253&  39 & 2$\cdot10^{-9}$ &  LP  \\

\\
MS\,1221.8$+$2452  & LAB  & 2.25$\pm$0.01 & 0.366$\pm$0.005 & 1.563/241&   90&  1$\cdot10^{-16}$ & LP  \\
                   & DL   & 2.25$\pm$0.01 & 0.367$\pm$0.003 & 1.561/241&   89&  1$\cdot10^{-16}$ & LP  \\
                   & Will & 2.25$\pm$0.01 & 0.368$\pm$0.003 & 1.533/241&   84&  1$\cdot10^{-16}$ & LP  \\
                   & free & 2.47$\pm$0.03 & 0.438$\pm$0.009 & 1.112/240&    1&  0.2              & PO  \\

\\
4C\,$+$21.35       & LAB  & 1.69$\pm$0.01 & 0.068$\pm$0.001 & 1.763/375& 267 & 1$\cdot10^{-16}$ &  LP  \\
                   & DL   & 1.69$\pm$0.01 & 0.068$\pm$0.001 & 1.795/375& 276 & 1$\cdot10^{-16}$ &  LP  \\
                   & Will & 1.70$\pm$0.01 & 0.068$\pm$0.001 & 1.802/375& 278 & 1$\cdot10^{-16}$ &  LP  \\
                   & free & 1.60$\pm$0.02 & 0.063$\pm$0.001 & 1.349/374& 123 & 1$\cdot10^{-16}$ &  LP  \\
\\
3C\,279            & LAB  & 1.54$\pm$0.01 & 0.240$\pm$0.001 & 1.293/608& 102& 1$\cdot10^{-16}$ &  LP  \\
                   & DL   & 1.55$\pm$0.01 & 0.242$\pm$0.001 & 1.260/608&  83 & 1$\cdot10^{-16}$ &  LP  \\
                   & Will & 1.55$\pm$0.01 & 0.242$\pm$0.001 & 1.259/608&  84 & 1$\cdot10^{-16}$ &  LP  \\
                   & free & 1.61$\pm$0.01 & 0.257$\pm$0.002 & 1.152/607&  25 & 7$\cdot10^{-7}$ &  LP  \\
\\
H\,1426$+$428      & LAB  & 1.90$\pm$0.01 & 1.373$\pm$0.005 & 1.678/584& 204 & 1$\cdot10^{-16}$ &  LP  \\
                   & DL   & 1.91$\pm$0.01 & 1.390$\pm$0.005 & 1.583/584& 159 & 1$\cdot10^{-16}$ &  LP  \\
                   & Will & 1.90$\pm$0.01 & 1.374$\pm$0.005 & 1.667/584& 199 & 1$\cdot10^{-16}$ &  LP  \\
                   & free & 1.99$\pm$0.01 & 1.498$\pm$0.011 & 1.317/583&  34 & 1$\cdot10^{-8}$ &  LP  \\
\\
PKS\,1424$+$240    & LAB  & 2.52$\pm$0.01 & 0.245$\pm$0.002 & 1.498/268&   104& 1$\cdot10^{-16}$ & LP  \\
                   & DL   & 2.50$\pm$0.01 & 0.243$\pm$0.002 & 1.560/268&   116& 1$\cdot10^{-16}$ & LP  \\
                   & Will & 2.54$\pm$0.01 & 0.250$\pm$0.002 & 1.384/268&    83& 1$\cdot10^{-16}$ & LP  \\
                   & free & 2.73$\pm$0.02 & 0.285$\pm$0.004 & 0.966/267&   0.4& 0.5              & PO  \\
\\
PKS\,1510$-$089    & LAB  & 1.34$\pm$0.01 & 0.107$\pm$0.001 & 1.096/661&  33 & 1$\cdot10^{-8}$ &  LP  \\
                   & DL   & 1.36$\pm$0.01 & 0.110$\pm$0.001 & 1.168/661&  68 & 1$\cdot10^{-15}$ &  LP  \\
                   & Will & 1.40$\pm$0.01 & 0.116$\pm$0.001 & 1.379/661& 166 & 1$\cdot10^{-16}$ &  LP  \\
                   & free & 1.29$\pm$0.01 & 0.102$\pm$0.001 & 1.032/660&   0.4 & 0.5 &  PO  \\
\\
PG\,1553$+$113     & LAB  & 2.28$\pm$0.01 & 1.023$\pm$0.004 & 1.405/433&  36 & 40$\cdot10^{-9}$ &  LP  \\
                   & DL   & 2.28$\pm$0.01 & 1.023$\pm$0.004 & 1.402/433&  36 & 5$\cdot10^{-9}$ &  LP  \\
                   & Will & 2.32$\pm$0.01 & 1.053$\pm$0.005 & 1.314/433&   10 & 2$\cdot10^{-3}$ &  LP  \\
                   & free & 2.35$\pm$0.01 & 1.084$\pm$0.010 & 1.288/432&   0.3 & 0.6 &  PO  \\
\\
1ES\,1959$+$650    & LAB  & 2.06$\pm$0.01 & 6.950$\pm$0.036 & 2.116/467& 316 & 1$\cdot10^{-16}$ &  LP  \\
                   & DL   & 2.08$\pm$0.01 & 7.082$\pm$0.037 & 1.967/467& 281 & 1$\cdot10^{-16}$ &  LP  \\
                   & Will & 2.29$\pm$0.01 & 8.676$\pm$0.046 & 1.329/467&   0.3 & 0.6 &  PO  \\
                   & free & 2.26$\pm$0.01 & 8.448$\pm$0.100 & 1.317/466&  22 & 3$\cdot10^{-6}$ &  LP  \\


\hline
\end{tabular}
\end{table*}




%%%%%%%%%%%%%%%%%%
% PAGE 2
%%%%%%%%%%%%%%%%%%

\clearpage
\newpage

\begin{table*}

\contcaption{}

%\label{table_fitpar_po}

\centering

\begin{tabular}{rccccccc}

\hline
(1)    & (2) & (3) & (4) & (5) & (6)  & (7)  & (8) \\
\hline
PKS\,2005$-$489    & LAB  & 2.47$\pm$0.01 & 0.927$\pm$0.006 & 0.990/327&   3 &  0.1 &  PO  \\
                   & DL   & 2.53$\pm$0.01 & 0.970$\pm$0.006 & 1.083/327&  30 & 1$\cdot10^{-7}$ &  LP  \\
                   & Will & 2.51$\pm$0.01 & 0.955$\pm$0.006 & 1.040/327&  18 & 3$\cdot10^{-5}$ &  LP  \\
                   & free & 2.44$\pm$0.02 & 0.911$\pm$0.011 & 0.986/326&   0.7 & 0.4 &  PO  \\
\\
PKS\,2155$-$304    & LAB  & 2.40$\pm$0.02 & 3.671$\pm$0.037 & 1.261/209&  21 & 9$\cdot10^{-6}$ &  LP  \\
                   & DL   & 2.41$\pm$0.02 & 3.704$\pm$0.037 & 1.239/209&  17 & 4$\cdot10^{-5}$ &  LP  \\
                   & Will & 2.41$\pm$0.02 & 3.690$\pm$0.037 & 1.248/209&  19 & 2$\cdot10^{-5}$ &  LP  \\
                   & free & 2.53$\pm$0.03 & 4.013$\pm$0.085 & 1.153/208&   1 & 0.2 &  PO  \\
\\
BL\,Lacertae       & LAB  & 1.50$\pm$0.01 & 0.267$\pm$0.002 & 2.002/616& 444 & 1$\cdot10^{-16}$ &  LP  \\
                   & DL   & 1.58$\pm$0.01 & 0.294$\pm$0.002 & 1.452/616& 182 & 1$\cdot10^{-16}$ &  LP  \\
                   & Will & 1.76$\pm$0.01 & 0.366$\pm$0.002 & 1.172/616&  15 & 1$\cdot10^{-4}$ &  LP  \\
                   & free & 1.71$\pm$0.01 & 0.344$\pm$0.004 & 1.121/615&   6 & 0.01 &  PO  \\
\\
B3\,2247$+$381     & LAB  & 2.19$\pm$0.01 & 0.350$\pm$0.005 & 1.632/283&  164&  1$\cdot10^{-16}$ & LP  \\
                   & DL   & 2.27$\pm$0.01 & 0.379$\pm$0.003 & 1.304/283&   79&  1$\cdot10^{-16}$ & LP  \\
                   & Will & 2.40$\pm$0.01 & 0.427$\pm$0.004 & 1.055/283&   10&  1$\cdot10^{-3}$  & LP  \\
                   & free & 2.46$\pm$0.03 & 0.449$\pm$0.010 & 1.035/282&    5&  0.03             & PO  \\
\\
1ES\,2344$+$514    & LAB  & 1.99$\pm$0.01 & 0.515$\pm$0.003 & 1.473/532& 195 & 1$\cdot10^{-16}$ &  LP  \\
                   & DL   & 2.04$\pm$0.01 & 0.546$\pm$0.003 & 1.247/532&  76 & 1$\cdot10^{-16}$ &  LP  \\
                   & Will & 2.26$\pm$0.01 & 0.687$\pm$0.004 & 1.572/532& 108 & 1$\cdot10^{-16}$ &  LP  \\
                   & free & 2.11$\pm$0.01 & 0.589$\pm$0.007 & 1.142/531&  31 & 3$\cdot10^{-8}$ &  LP  \\




                   


\hline
\end{tabular}
\end{table*}

